One-Time Compilation of Device-Level Instructions for Quantum Subroutines

A large class of problems in the current era of quantum devices involve interfacing between the quantum and classical system. These include calibration procedures, characterization routines, and variational algorithms. The control in these routines iteratively switches between the classical and the quantum computer. This results in the repeated compilation of the program that runs on the quantum system, scaling directly with the number of circuits and iterations. The repeated compilation results in a significant overhead throughout the routine. In practice, the total runtime of the program (classical compilation plus quantum execution) has an additional cost proportional to the circuit count. At practical scales, this can dominate the round-trip CPU-QPU time, between 5% and 80%, depending on the proportion of quantum execution time. To avoid repeated device-level compilation, we identify that machine code can be parametrized corresponding to pulse/gate parameters which can be dynamically adjusted during execution. Therefore, we develop a device-level partial-compilation (DLPC) technique that reduces compilation overhead to nearly constant, by using cheap remote procedure calls (RPC) from the QPU control software to the CPU. We then demonstrate the performance speedup of this on optimal pulse calibration, system characterization using randomized benchmarking (RB), and variational algorithms. We execute this modified pipeline on real trapped-ion quantum computers and observe significant reductions in compilation time, as much as 2.7x speedup for small-scale VQE problems.

==> content/00_outline.tex <==
\section{Introduction}
Introduce and motivate the problem. Give a glimpse into the proposed solution.
\begin{itemize}
    \item What is VQE, and why is it important in the NISQ-era of device.
    \item Why is compilation a bottleneck for VQE
    \item Time and cost estimates of compilation (Gu et al)
    \item Problems solved by people in compilation - eg: Qiskit Runtime, Pranav pulse partial compilation
    \item What is the problem we solve
    \item Advantage with state-of-the-art VQE, i.e., ADAPT
\end{itemize}
\section{Background}
\begin{itemize}
    \item Quantum Computing
    \item VQE with classic VQE diagram
    \item Compilation for VQE - important to drill down on the problem we are addressing
    \begin{itemize}
        \item What the field understands by compilation
        \item Divide into upstream and downstream
        \item We fix the downstream compilation
        \item Other works focus on upstream
    \end{itemize}
    \item ARTIQ control system
\end{itemize}
\section{Related Work}
\begin{itemize}
    \item Qiskit Runtime
    \item Pranav's paper
    \item Potentially Andi Gu et al paper?!
\end{itemize}
\section{Current Compilation Method}
\begin{itemize}
    \item Circuit executed on kernel
    \item Optimization done on host
    \item Context switches between host and kernel every iteration
\end{itemize}
\section{New Compilation Method}
\begin{itemize}
    \item Control always stays in a kernel that is opened only once
    \item Use RPC to talk to host and get new parameters
    \item New parameters accessed using multi-threaded structure
\end{itemize}
\section{Experimental Results}
Talk about results we got from running on an actual system.
\begin{itemize}
    \item What is STAQ
    \item What experiment did we run on STAQ
    \item What does the data look like
    \item How much overhead do we save
\end{itemize}
\section{Discussion}
Discuss how the advantage would scale, and where does our advanatge grow
\begin{itemize}
    \item What do compile times looks like for larger number of gates, qubits, shots
    \item What is the advantage of our method
    \begin{itemize}
        \item In the worst case we always have a k\% advantage, where k depends on circuit runtime
        \item Talk about how better hardware and research on shot budget helps us
        \item Quantitative cost by bringing in Gu et al paper
        \item Added advantage with protocols like ADAPT
    \end{itemize}
\end{itemize}


==> content/30_motivation.tex <==
\section{Motivation}
\label{sec:motivation}

% Quantum computers require significant amounts of setup before they are operational for computation. For every type of underlying hardware
% % , for example superconducting qubits, trapped ions, or neutral atoms, 
% the device must be extensively characterized and its operations calibrated. Such routines, similar to variational algorithms, require constant interaction between the quantum and classical processing, i.e. there is no single shot pass which prepares the hardware into a runnable state. Multiple rounds of circuit preparation, execution, and subsequent classical post-processing are performed, which can incur significant compilation overhead.
% % Like variational or other interactive applications, repeated cyclic behavior incurs significant kernel start-up and compilation overheads.
The runtime of a quantum program involves compilation time and execution time. The execution time is often divided between classical execution on the \ac{cpu} and quantum execution on the \ac{qpu}, with varying ratios based on the type of program. In today's landscape of quantum computing, users submit programs to cloud-hosted quantum systems using a job queue. Device-level compilation for every single job on this queue can add significant overhead. Outside of this general case, a similar compilation overhead problem is also incurred when running \ac{qci} problems where control flow iteratively changes from the classical system to the quantum system resulting in repeated compilation. This compilation overhead motivates the need for a new model of execution for quantum programs that compiles to the \ac{qpu} only once and streams the execution of subsequent programs without the need for recompilation. This is possible only if a shared structure can be identified between programs/executions and each run executed as a different parametric version of this shared structure. High-level representations of programs vary widely, and a shared structure is apparent only when these high-level programs are reduced to low-level hardware specific representations, or \emph{device-level representations}. As a result we focus on enabling this through \ac{dlpc}.
% In this section, we further motivate the need for our partial-compilation technique for classes of calibration, characterization, and applications which depend on \ac{qci} routines. A sample schematic for these routines can be seen in Fig.~\ref{fig:qci_programs}.

% A quantum computer has to go through preparatory routines before it can run programs corresponding to interesting applications. Some of these preparatory routines include calibration and characterization of the system. Both of these routines require the classical computer to work in tandem with the quantum system. In this section we motivate our partial-compilation technique by outlining examples of calibration, characterization and applications which involve \ac{qci} routines.

% \subsection{Optimized Calibration}
% \label{subsec:calib}
% Quantum computers require high fidelity (low error) state preparation, operations, and measurements. The parameters of a quantum system drift with time resulting in systematic errors that affect the fidelities. This motivates the need for periodic calibration of the system to appropriately adjust gate pulse parameters. A naive scan across parameters to re-calibrate the system can be expensive, and there have been recent proposals to make these calibration routines optimal~\cite{Majumder2020, PhysRevA.102.042611, Maksymov_2021, stace2022optimised}. These calibration routines involve quantum-classical interfacing, requiring analysis and computation on the classical computer every iteration as it attempts to converge to the optimal pulse parameters. This adds an overhead associated with recompiling the pulse sequence every iteration. In general, calibration procedures do not calibrate operations on all N qubits of the system simultaneously,
% and instead characterize subsets, e.g. every pair of connected
% qubits, which requires an additional factor of $O(N^2)$ machine
% compilations. In this work, we explore Stace, et al.'s proposal on using Bayesian inference for optimizing pulse sequences~\cite{stace2022optimised} as an example to demonstrate the compilation overhead. Their work shows the calibration of single and two-qubit gate pulse sequences using a Bayesian inference model on the classical computer, 
% % Their proposal optimizes 2 parameters for single-qubit operations and 5 parameters for two-qubit entangling operations, both of which are
% realized using piece-wise constant amplitude-modulated pulse sequences. Because these calibration routines operate at the level of pulses, the only relevant layers from the compilation pipeline here are pulse-level and device-level compilation. The pulse-level compilation here adds no overhead as there is no optimization being performed, instead these routines are used to find the optimal pulse for the given system. Device-level compilation, however, is required to compile the pulses down to executable binaries which by default is done each cycle. 

% % Our partial-compilation technique focuses on device-level compilation, optimal calibration routines lend themselves as an ideal target for our proposed method. Section~\ref{sec:results} shows the estimated compilation overhead of Stace, et al's optimization technique, and compares it to our proposed partial-compilation technique.

% \subsection{System Characterization}
% \label{subsec:charac}
% System characterization refers to routines that are run on a quantum computer to assess the noise in the system and are often used in conjunction with calibration. Widely used characterization routines include \ac{gst}~\cite{https://doi.org/10.48550/arxiv.1310.4492}, \ac{rb}~\cite{PhysRevA.77.012307, magesan2011scalable}, cycle benchmarking~\cite{Erhard2019}, and empirical direct characterization~\cite{dahlhauser2022benchmarking}. Most of these routines involve sequential execution of series of generated circuits, 
% % and while they do not necessarily require this circuit execution to be interleaved with classical computation there is still
% with a significant overhead associated with compiling large numbers of circuits each to be run only a few times on the quantum computer. We focus on \ac{rb} as an illustrative example of the present device-compilation overhead. \ac{rb} runs circuits with increasingly longer sequences of randomly generated gates \cite{PhysRevA.77.012307}.
% % The general idea of \ac{rb} can be summarized as follows. For a given length, $l$, a series of circuits with $l$ gates are generated by randomly sampling from a set of gates operating on the number of qubits in the system. These circuits are then sequentially executed on the quantum computer, resulting in an effective unitary $U$. This is followed by a unitary $U^{\dagger}$ which brings the system back to its initial state \cite{PhysRevA.77.012307}. 
% % This is repeated for increasing sequence lengths $l$. A comprehensive outline of this routine can be found at~\cite{PhysRevA.77.012307}. 
% % Although this routine, along with other characterization algorithms, do not strictly fall into the class of \ac{qci} problems, they do involve repeated compilation of circuits. 
% Similar to calibration, system operators characterize subsets, e.g. every pair of connected qubits, resulting in an additional factor of $O(N^2)$ machine compilations~\cite{Helsen2019}.
% % In the best case, it is preferable to sample \textit{more circuits} rather than \textit{more samples per circuit} meaning the actual time spent on the \ac{qpu} is relatively small.  

% % Given that the circuits that are run as part of these algorithms are targeted primarily towards benchmarking, generated circuits are run as is, and the pulses that correspond to the operations in these circuits have been pre-optimized for each operation. This results in no significant gate and pulse-level compilation, with device-level compilation then being the bottleneck in their compilation pipeline. 
% % In an example like \ac{rb}, where this routine can be repeated for sequence lengths on the order of $10^{2}$, the cost of compiling each circuit can be significant. 
% % We discuss how our proposed technique reduces the device-level compilation overhead for characterization routines in Section~\ref{sec:fast}, and demonstrate the results of the speedup in Section~\ref{sec:results}.

% \subsection{Variational Quantum Eigensolver}
% \label{subsec:vqe}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/kernel_flow.pdf}
%     % \vspace{-1\baselineskip}
%     \caption{Kernel execution of parameterized quantum operations. Consider a gate $U$ acting on qubit $q$ with a parameter $\theta$. First, the hardware-specific qubit invariants are retrieved from the persistent dataset. Here, invariant parameters are the qubit frequency $\omega$, Rabi frequency $\Omega$, and phase associated with the gates $\phi$. The desired pulse is configured by setting $\omega$ with a offset $\phi$ on the direct digital synthesizer (DDS), and $\Omega$ and the gate parameter $\theta$ are used to calculate the pulse duration, here from \cite{kim2020hardware}. The DDS plays the appropriate pulse sequence for the dynamically and analytically calculated duration. The kernel can be compiled just once with the invariant parameters, while the variables are supplied during runtime at each iteration.}
    
%     % The single-qubit example here uses qubit parameters and pulse times from demonstrations on the quantum computer described in~\cite{kim2020hardware}. In this example, we consider a single-qubit parameterized circuit being repeated with different angles $\theta_{1}$ and $\theta_{2}$ at each iteration. It is observed that the only change in the executable at runtime is the pulse duration which is analytically computed quickly. This observation allows the kernel to be compiled just once with the invariant parameters, while the variables are supplied during runtime at each iteration, thereby saving on re-compilation costs.}
%     % \vspace{-\baselineskip}
%     \label{fig:kernel_flow}
% \end{figure*}
% For near-term quantum devices, a promising application is \ac{vqe}.
% % This problem is considered to be exponentially hard to solve using a classical machine but can potentially be solved efficiently using a quantum computer. \ac{vqe} was developed as an alternative to \ac{qpe}, which is also capable of solving the same problem ~\cite{lloyd_qpe} but in a variational way rather than directly. Given the current error rates and number of qubits  available, \ac{qpe} is not a feasible algorithm in the \ac{nisq} era of quantum devices. For a given precision $\epsilon$, \ac{qpe} requires $O(1)$ repetitions of depth $O(1/\epsilon)$ circuits, while \ac{vqe} requires $O(1/\epsilon^{2})$ repetitions of depth $O(1)$ circuits ~\cite{Wang_2019}.
% \ac{vqe} is a hybrid, iterative algorithm that uses the variational method~\cite{griffiths_schroeter_2018} and can be used to find the ground state energy of a molecule~\cite{Peruzzo2014}. 
% % This is done by constructing a Hamiltonian whose minimum expectation value approximates the ground state energy of the molecule. 
% A Hamiltonian (essentially a large paramterized matrix) is a quantum mechanical operator which corresponds to the total energy of a system. A parameterized quantum circuit, or ansatz, with measurements corresponding to the constructed Hamiltonian is then iteratively executed with varying parameters until the expected value of the Hamiltonian converges to the optimal value. On each iteration, the next set of parameters and set of measurements for the circuit are determined by a classical optimizer which runs on the \ac{cpu}, as opposed to the ansatz circuit, which is executed on the \ac{qpu}. %This routine of a classical optimizer working in tandem with the execution of quantum circuits makes \ac{vqe} a hybrid algorithm.%

% At the gate-level, a \ac{vqe} program remains invariant with respect to the type of gates being used across iterations. However, the changing parameters of these gates over each iteration have cascading effects on the resultant pulses and device-level code. In the naive pipeline, this results in these components being re-compiled every iteration. Past work, like \cite{gokhale_variational}, propose compiler optimizations and partial compilation techniques to reduce the pulse-level re-compilation overhead. In Section~\ref{sec:results} we show that for real small-scale systems the device-level compilation time can be significant, and demonstrate how our proposed routine reduces this overhead to being nearly constant.
